IBCB: Efficient Inverse Batched Contextual Bandit for Behavioral Evolution History

Traditional imitation learning focuses on modeling the behavioral mechanisms of experts, which requires a large amount of interaction history generated by some fixed expert. However, in many streaming applications, such as streaming recommender systems, online decision-makers typically engage in online learning during the decision-making process, meaning that the interaction history generated by online decision-makers includes their behavioral evolution from novice expert to experienced expert. This poses a new challenge for existing imitation learning approaches that can only utilize data from experienced experts. To address this issue, this paper proposes an inverse batched contextual bandit (IBCB) framework that can efficiently perform estimations of environment reward parameters and learned policy based on the expert's behavioral evolution history. Specifically, IBCB formulates the inverse problem into a simple quadratic programming problem by utilizing the behavioral evolution history of the batched contextual bandit with inaccessible rewards. We demonstrate that IBCB is a unified framework for both deterministic and randomized bandit policies. The experimental results indicate that IBCB outperforms several existing imitation learning algorithms on synthetic and real-world data and significantly reduces running time. Additionally, empirical analyses reveal that IBCB exhibits better out-of-distribution generalization and is highly effective in learning the bandit policy from the interaction history of novice experts.

==> Sections/experiment/results_ablation.tex <==
% \subsection{Ablation Study: Summary}
% \subsubsection{Detailed Results of Out-of-distribution Data on Synthetic Dataset}
% \\ %-- \ref{app:exp:details:ab:ML}.\\
%In this subsection, we discussed several extreme situations (mentioned in Introduction \ref{intro}) that imitation learning (IL) algorithms and IBCB may face with. Training logs (expert's behavioral evolution history) may update in a delayed manner in online learning, which means that when training models, we may only have access to former part of expert's behavioral evolution history data (e.g. IL and IBCB can only obtained the former half part of the data, but original expert has evolved with the whole training data), and contradictory data may appear. Since that original expert policy's hyper parameter ($\alpha$ in Algorithm \ref{alg:CBB:bandit:TS}, detailed settings shown in Appendix \ref{app:exp:details:train:expert}) is also inaccessible for IBCB, we also checked the influence of IBCB's hyper parameter's ($\alpha$ in \eqref{eq:inverse:opt:constriant} ) setting. Detailed results and analyses of IBCB's hyper parameter test on syntheic dataset and the whole ablation study on ML-100K dataset can be found in Appendix~\ref{app:exp:details:param} and \ref{app:exp:details:ab:ML}.\\ %Note that large scale contradictory data rarely shown in real world, contradictory data test was only done on synthetic dataset. Since we set the right-hand side of \eqref{eq:inverse:opt:constriant} to 0 when we assume expert is SBTS, IBCB's hyper parameter test was only done on SBUCB backbone.  %Specifically, we set $\alpha$ to be 1(original), 0.6, 0.8, 1.2, 1.5 and 2 to check whether $\alpha$ setting of the \eqref{eq:inverse:opt:constriant} will significantly influence the whole performance or not. Note that this setting was suitable for experiments based on SBUCB backbone since $\alpha=0$ when original model's backbone is SBTS.
% \begin{table}[!ht]
%     \centering
%     \setlength{\abovecaptionskip}{3pt}
%     \setlength{\belowcaptionskip}{-3pt}
%     \caption{Reward parameters' estimation on synthetic dataset (using first half of expert's behavior evolution history logs). BaseSVC cannot obtain reward parameters, so it was excluded from OL-Fitness comparison.}
%     \resizebox{!}{0.9cm}{
%     \begin{tabular}{l|c|c|c|c}
%         %\toprule[1.5pt]
%         \hline
%         \multirow{2}{*}{Algorithm} & \multicolumn{4}{c}{Online Train Log Fitness (Half Train)} \\
%         \cline{2-5} ~ & std=0 & std=0.03 & std=0.07 & std=0.10  \\ 
%         \hline \hline
%         %\midrule[1.5pt]
%         SBUCB & \textcolor[rgb]{0,0,0}{0.883±0.007} & \textcolor[rgb]{0,0,0}{0.879±0.016} & \textcolor[rgb]{0,0,0}{0.878±0.018} & \textcolor[rgb]{0,0,0}{0.874±0.019}  \\
%         \hline
%         B-IRL & {0.752±0.018} & {0.729±0.051} & {0.728±0.050} & {0.721±0.047}  \\ 
%         B-ICB-S & 0.730±0.039 & 0.727±0.045 & 0.721±0.063 & 0.717±0.041  \\
%         %\midrule
%         \hline
%         IBCB (Ours) & \textbf{\textcolor[rgb]{0,0,0}{0.895±0.011}} & \textbf{\textcolor[rgb]{0,0,0}{0.894±0.016}} & \textbf{\textcolor[rgb]{0,0,0}{0.892±0.024}} & \textbf{\textcolor[rgb]{0,0,0}{0.886±0.017}}  \\ 
%         %\bottomrule[1.5pt]
%         \hline
%     \end{tabular}
%     }  
%     %\caption{real environment parameter's estimation}
%     % \label{tab:ab:ce:real:env:val}
%     % \caption{Reward parameters' estimation on synthetic dataset (using first half of expert's behavior evolution history logs). BaseSVC cannot obtain reward parameters, so it was excluded from OL-Fitness comparison.}
%     \label{tab:ab:ce:real:env:val:tot}
% \end{table}
% %bt test (ce)
% \begin{table}[!ht]
%     \centering
%     \setlength{\abovecaptionskip}{3pt}
%     \setlength{\belowcaptionskip}{-3pt}
%     \caption{{Expert policy parameters' estimation on synthetic dataset (using first half of expert's behavioral evolution history logs). Expert policy produces same actions compared with itself, so BT-Fitness of expert policy is 1.}}
%     % \begin{subtable}[ht]{1\linewidth}
%     % \centering
%     \resizebox{!}{1.2cm}{
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{l|c|c|c|c}
%         %\toprule[1.5pt]
%         \hline
%         \multirow{2}{*}{Algorithm} & \multicolumn{4}{c}{Batch Test Log Fitness (Half Train)} \\
%         \cline{2-5} ~ & std=0 & std=0.03 & std=0.07 & std=0.10 \\ 
%         %\midrule[1.5pt]
%         \hline \hline
%         SBUCB & \textcolor[rgb]{0,0,0}{1} & \textcolor[rgb]{0,0,0}{1} & \textcolor[rgb]{0,0,0}{1} & \textcolor[rgb]{0,0,0}{1} \\ 
%         \hline
%         B-IRL & {0.718±0.012} & {0.699±0.031} & {0.702±0.035} & {0.694±0.037} \\ 
%         BaseSVC & 0.656±0.019 & 0.638±0.039 & 0.638±0.043 & 0.627±0.045 \\ 
%         B-ICB-S & 0.695±0.054 & 0.707±0.069 & 0.695±0.084 & 0.688±0.043 \\ 
%         %\midrule
%         \hline
%         \textbf{IBCB (Ours)} & \textbf{\textcolor[rgb]{0,0,0}{0.891±0.019}} & \textbf{\textcolor[rgb]{0,0,0}{0.919±0.030}} & \textbf{\textcolor[rgb]{0,0,0}{0.890±0.031}} & \textbf{\textcolor[rgb]{0,0,0}{0.890±0.023}} \\ 
%         %\bottomrule[1.5pt]
%         \hline
%     \end{tabular}
%     }
%     % \label{tab:ab:ce:bt:bandit:SBUCB:fitness}
%     % \end{subtable}

%     \vspace{1em}

%     % \begin{subtable}[ht]{1\linewidth}
%     % \centering
%     \resizebox{!}{1.2cm}{
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{l|c|c|c|c}
%         %\toprule[1.5pt]
%         \hline
%         \multirow{2}{*}{Algorithm} & \multicolumn{4}{c}{Batch Test Average Reward (Half Train)}\\
%         \cline{2-5} ~ & std=0 & std=0.03 & std=0.07 & std=0.10 \\ 
%         %\midrule[1.5pt]
%         \hline \hline
%         SBUCB & \textcolor[rgb]{0,0,0}{0.641±0.010} & \textcolor[rgb]{0,0,0}{0.629±0.028} & \textcolor[rgb]{0,0,0}{0.630±0.024} & \textcolor[rgb]{0,0,0}{0.622±0.024}  \\ 
%         \hline
%         B-IRL & 0.545±0.020 & 0.522±0.047 & 0.522±0.046 & 0.510±0.046  \\ 
%         BaseSVC & 0.520±0.023 & 0.497±0.053 & 0.497±0.052 & 0.482±0.051 \\ 
%         B-ICB-S & {0.549±0.019} & {0.538±0.024} & {0.540±0.030} & {0.529±0.033} \\ 
%         %\midrule
%         \hline
%         \textbf{IBCB (Ours)} & \textbf{\textcolor[rgb]{0,0,0}{0.610±0.015}} & \textbf{\textcolor[rgb]{0,0,0}{0.608±0.025}} & \textbf{\textcolor[rgb]{0,0,0}{0.597±0.036}} & \textbf{\textcolor[rgb]{0,0,0}{0.588±0.030}}  \\ 
%         %\bottomrule[1.5pt]
%         \hline
%     \end{tabular}
%     }
%     % \label{tab:ab:ce:bt:bandit:SBUCB:AR}
%     % \end{subtable}
%     % \caption{{Expert policy parameters' estimation on synthetic dataset (using first half of expert's behavioral evolution history logs). Expert policy produces same actions compared with itself, so BT-Fitness of expert policy is 1.}}
%     \label{tab:ab:ce:bt:bandit:SBUCB:tot}
% \end{table}
%dup test
%we also made duplicated data test in the following part.

% Table~\ref{tab:ab:ce:real:env:val:tot}--Table~\ref{tab:ab:param:bt:bandit:SBUCB:tot} in Section~\ref{app:exp:details:dup} present main ablation study results on synthetic dataset. Key findings include: (1) When limited to the first half of the expert's logs, IBCB still outperforms IL baselines, showing less performance degradation compared to the full data scenario in Tables \ref{tab:real:env:val:tot} and \ref{tab:bt:bandit:SBUCB:tot}. (2) Contradictory data significantly affects BaseSVC's fitness but does not impact models that learn reward parameters like IBCB, highlighting IBCB's robustness in extreme conditions.
%Table~\ref{tab:ab:ce:real:env:val:tot}--Table~\ref{tab:ab:dup} reports the results of different ablation studies (exclude IBCB's hyper parameter test, see details in Appendix~\ref{app:exp:details:param}) on synthetic dataset. We have the following observations: (1) When all IL baselines and IBCB only have the access to the first half of expert's behavioral evolution history logs, \textit{i.e., novice expert's evolution history}, IBCB can have better performance, compared with the degree of decline in all algorithms from Table~\ref{tab:real:env:val:tot} and Table~\ref{tab:bt:bandit:SBUCB:tot}. (2) Contradictory data undermines BaseSVC's (BC model) fitness on expert's behavior evolution history and BT-Fitness, but models which learns reward parameters, including IBCB, are not influenced by this phenomenon, which demonstrate IBCB's robustness for extreme situations.

% \input{Sections/appendix/appendix_result_details}
